CoNav Chair: Design of a ROS-based Smart Wheelchair for Shared Control Navigation in the Built Environment

With the number of people with disabilities (PWD) increasing worldwide each year, the demand for mobility support to enable independent living and social integration is also growing. Wheelchairs commonly support the mobility of PWD in both indoor and outdoor environments. However, current powered wheelchairs (PWC) often fail to meet the needs of PWD, who may find it difficult to operate them. Furthermore, existing research on robotic wheelchairs typically focuses either on full autonomy or enhanced manual control, which can lead to reduced efficiency and user trust. To address these issues, this paper proposes a Robot Operating System (ROS)-based smart wheelchair, called CoNav Chair, that incorporates a shared control navigation algorithm and obstacle avoidance to support PWD while fostering efficiency and trust between the robot and the user. Our design consists of hardware and software components. Experimental results conducted in a typical indoor social environment demonstrate the performance and effectiveness of the smart wheelchair hardware and software design. This integrated design promotes trust and autonomy, which are crucial for the acceptance of assistive mobility technologies in the built environment.

==> contribution.tex <==
\section{Research Objectives and Contributions}
\label{sec:contribution}
\par 

Building on insights from previous smart wheelchair designs and shared control-based navigation structures, we developed both the hardware and software for a shared control-based smart wheelchair. On the hardware side, we created a differential drive-based wheelchair model equipped with multiple integrated sensors, including LiDAR, a camera, an IMU, and encoders. This multi-sensor setup enables the wheelchair to perceive its surroundings in real-time, facilitating precise and responsive movements. On the software side, we implemented a shared control-based navigation system~\cite{xu2024} that allows the wheelchair to navigate effectively while adapting to the user's control inputs. This system enhances the interaction between the user and the robot, fostering greater trust and cooperation. Generally speaking, this hardware and software design solved two parts of the challenge from the side of PWD and smart wheelchair development.

In general, our proposed system has the following contribution:
\begin{itemize}
    \item We have developed a multi-sensor based smart wheelchair hardware platform to enhance the mobility and independence of users, providing a reliable and user-friendly solution to those with mobility impairments.
    \item We propose a novel shared control-based navigation framework for assistive mobile robots integrating a user’s desire for path preference and control during navigation to improve the efficiency and human-robot trust.
    \item We have tested our wheelchair system in a built environment and demonstrate that our robot system outperforms other autonomous wheelchair navigation systems both in effectiveness and user’s comfort. 
\end{itemize}
